Longitudinal Study of an IP Geolocation Database

IP geolocation - the process of mapping network identifiers to physical locations - has myriad applications. We examine a large collection of snapshots from a popular geolocation database and take a first look at its longitudinal properties. We define metrics of IP geo-persistence, prevalence, coverage, and movement, and analyse 10 years of geolocation data at different location granularities. Across different classes of IP addresses, we find that significant location differences can exist even between successive instances of the database - a previously underappreciated source of potential error when using geolocation data: 47% of end users IP addresses move by more than 40 km in 2019. To assess the sensitivity of research results to the instance of the geo database, we reproduce prior research that depended on geolocation lookups. In this case study, which analyses geolocation database performance on routers, we demonstrate impact of these temporal effects: median distance from ground truth shifted from 167 km to 40 km when using a two months apart snapshot. Based on our findings, we make recommendations for best practices when using geolocation databases in order to best encourage reproducibility and sound measurement.

==> Makefile <==
.PHONY : fig

.SUFFIXES: _table.tex _table_scaled.tex .pdf _cropped.pdf

MAIN=paper
BIBS=geo.bib
PDFTEX=pdflatex
BIBTEX=bibtex

FIGS=		

SRCS=$(MAIN).tex intro.tex survey.tex methodology.tex \
	evaluation.tex usecases.tex conclusion.tex appendix.tex \
	data.tex reverse.tex $(FIGS)

REFS=$(BIB).bib

all: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).tex $(BIBS) $(SRCS)
	$(PDFTEX) $(MAIN)
	$(BIBTEX) $(MAIN)
	$(PDFTEX) $(MAIN)
	$(PDFTEX) $(MAIN)

$(MAIN).html: $(MAIN).tex $(BIBS) $(SRCS)
	latex2html $(MAIN)

tidy:
	rm -f *.dvi *.aux *.log *.blg *.bbl

clean:
	rm -f *.dvi *.aux *.log *.blg *scaled.tex *.bbl $(MAIN).ps $(MAIN).pdf


==> reverse.tex <==
%RB: new section that looks at possible explaining factors
\section{Sources of Variation}

%\subsection{Limitations}

Our primary contribution in this work is to define rigorous metrics
for characterizing the dynamics of geolocation databases.  We keenly
recognize that location changes within the database may be real or
may be artifacts of the geolocation system's methodology.  For
instance, a database that utilizes new information to update a prefix
from a default location will present as a change, even when no change
has occurred.  Similarly, anycast can induce incorrect changes even 
when conflicting locations are all true instances of the addresses.
On the other hand, there is a rich ecosystem of IP transfer markets and
such transfers occur commonly~\cite{livandariu2017}.  These effects
all manifest in different ways in the \maxmind data.

In this section, we take a first step toward exploring potential
correlations with external data and common sources of error and
location changes.  However, we do
not investigate the root causes of the dynamics we observe.  Indeed,
we note that this limitation is fundamental --  \maxmind's algorithm is
proprietary so that we cannot provide true causal analysis.  
Rather, we focus on characterizing the widely used \maxmind
database and providing guidelines for how researchers should view and
utilize geodatabases.  

\subsection{Anycast}\label{sec:evaluation:anycast}
%\begin{figure}[h]
%% \centering
%\includegraphics[width=0.40\textwidth]{figures/distinct_anycast_cdf}
%\caption{Number .}
%\label{fig:anycast}
%\end{figure}
A special category of IP addresses within the geolocation
database we wish to study are anycast addresses.  Anycast is used
for load-balancing and resilience by addressing multiple
geographically and topologically disparate end points
with the same IP address.  IP routing then directs traffic to anycast
addresses to the topologically nearest instance.
%RB: add DNS anycast \cite
Anycast is frequently used in \eg DNS~\cite{sarat2006use}.
 
Anycast is particularly interesting in the context of IP geolocation
as the correct answer is a set of geolocations, or the geolocation
with respect to a particular client request.  To better understand the
way anycast addresses present in \maxmind, 
we use the publicly available dataset 
from Cilasece \etal~\cite{cicalese2018longitudinal} that 
surveys the anycast prefixes 
across the June 2016 to April 2017 period.  
The data consists of monthly lists of IP addresses labeled as anycast. 

As we did for 
end host infrastructure and router datasets,
we take the intersection of these monthly sets of IP addresses for 
a total of 2,552 IP addresses in 2,552 different /24. 
We find that these IP addresses have a single dominant country and city:
$>$ 99.9\% (99\%) of these IP addresses have a single
country (city) over all snapshots, whereas Cilasece \etal found that
there
were at least two instances of these addresses.
Compared to the mean maximum prevalence for all IP addresses at the 
city-level, the maximum prevalence for
anycast prefixes is much higher. 

\paragraph{\textbf{Lesson}}
We conclude that \textbf{\maxmind uses a ``default'' country and city for 
per anycast prefix}.

\subsection{Routed Address Coverage}\label{sec:evaluation:coverage}

\begin{figure}[!t]
\begin{subfigure}{.38\textwidth}
 \centering
\includegraphics[width=\linewidth]{metrics/coverage/coverage_full_country_with_jaccard.pdf}
 \caption{IPs with country geolocations}
 \label{fig:coverage-full-country-with-jaccard}
 \end{subfigure}%
 \begin{subfigure}{.38\textwidth}
  \centering
\includegraphics[width=\linewidth]{metrics/coverage/coverage_full_city_with_jaccard.pdf}
 \caption{IPs with city geolocations}
 \label{fig:coverage-full-city-with-jaccard}
 \end{subfigure}%
 \\
 \begin{subfigure}{.36\textwidth}
\includegraphics[width=\linewidth]{metrics/coverage/coverage_type_city.pdf}
 \caption{Coverage by address type}
 \label{fig:coverage-type-city}
 \end{subfigure}
 \vspace{-2mm}
 \caption{Understanding \maxmind coverage over time relative to BGP
          (Route Views) and Jaccard
          distance within years.  Many routed addresses are not 
          present in \maxmind, and city-level locations are volatile.}
  \label{fig:coverage-full-with-jaccard}
\end{figure}


%RB: this needs some more intro to differentiate it from previous
%subsection -- it's confusing b/c there's two types of "coverage"
%being discussed.  trying this; pls edit:
Next, we consider a different notion of coverage -- the coverage
relative to routed IP address space.  To assess routed
address space coverage, we utilize the global BGP tables available
from Route Views~\cite{routeviews} coinciding with the date of each
\maxmind snapshot.
Fig.~\ref{fig:coverage-full-with-jaccard} shows the coverage on stacked bars
over 10 years. For each year, we 
show the average numbers over the year of three types of information:  
IP addresses covered by \maxmind, advertised but missing in \maxmind, 
and present in \maxmind but not in the global BGP table.
We also show as a secondary Y-axis the Jaccard distance 
(Eq.~\ref{eq:jaccard-distance-coverage}) on all the snapshots of the year.

\subsubsection{Country}\label{sec:all-ip-bgp-country}
Fig.~\ref{fig:coverage-full-country-with-jaccard} shows
that from 2010 to 2019, there is an increasing 
number of IP addresses present in the database at the country-level,
following the general increase of IP space
announced in BGP. 
The Jaccard distance decreases over time, meaning that 
the set of IP addresses with a country listed in the database becomes
more stable 
over time. 

A closer look at the coverage at the country 
level for different type of IP address revealed that it does not depend on the type of IP address 
as the metricstays very close to one over the entire year.

\subsubsection{City}\label{sec:bgp-city}

At the city-level, we find dramatically different coverage results.
First, 
it is interesting
to note in Fig.~\ref{fig:coverage-full-city-with-jaccard} that \maxmind coverage is not correlated to Route Views. Indeed, 
the cumulative yellow and blue bars, corresponding to the
number of IP addresses announced in 
BGP, increases over time as expected.  However, the yellow bar alone does 
not increase
the same way; since 2017, it even decreases implying that the fraction
of addresses within the global BGP table without a city-level
geolocation in the database has decreased.

The Jaccard distance shows that city-level coverage for IP addresses
is volatile. In 2019, 35\% of IP addresses that had a city location
present in the database at least once also
had at least one snapshot where the city was not present.
Fig.~\ref{fig:coverage-type-city} shows two things: first, 
the overall coverage is relatively constant over time for all classes of IP addresses.
However, the coverage value strongly 
depends on the type of address. There is about 90\% coverage 
for end users, 37\% for end host infrastructure and 41\% for routers. 
The Jaccard distance is interesting: going from 0.16 
for end users, to 0.47 for routers. 
This means that even if the coverage is constant over time, the set of 
IP addresses covered varies significantly.

\paragraph{\textbf{Lesson}}
Looking at geolocation coverage
from 2010 to 2019, 
\textbf{almost all allocated IP addresses are present at the country
granularity}. However, 
in 2019, \textbf{fewer than half of the allocated IP addresses are
included in the city-level database}. Moreover, 
within that year, \textbf{the set of IP addresses with city
geolocations is highly variable}.


\subsection{Registry Information}

To gain a deeper understanding of coverage, we analyzed IP
address registry information.  While the construction of \maxmind's
database is private, it has been hypothesized that many databases fall
back on registry information when more granular data is unavailable.  We 
use registry information available via whois to analyze 3000 prefixes
corresponding to 
IP addresses announced 
in BGP but not covered by \maxmind at the country level. 
% So we used present whois information to do 
% this analysis, because I couldn't find  whowas API common for all RIRs. 

Interestingly, we find that there was no dominant characteristic or
readily ascertainable correlation among these prefixes.
The prefixes were distributed over 2,038 different AS and 
over 114 countries in \maxmind. 
%For the converse case of IP addresses covered by \maxmind but not announced in 
%BGP, the non negligible number of this type of IP address reinforces our belief
%that \maxmind does have privileged feeds 
In the converse case of the 19,637 prefixes covered by \maxmind but not
announced in BGP, we find that only 
9.3\% of these addresses had registry information in the whois.  

%\begin{figure}[!t]
%\begin{subfigure}{.40\textwidth}
%\centering
%\includegraphics[width=\linewidth]{metrics/coverage/coverage_type_country.pdf}
% \caption{Country}
% \label{fig:coverage-type-country}
%\end{subfigure}%
% \begin{subfigure}{.40\textwidth}
%\includegraphics[width=\linewidth]{metrics/coverage/coverage_type_city.pdf}
% \caption{City}
% \label{fig:coverage-type-city}
% \end{subfigure}
% \vspace{-2mm}
% \caption{Coverage by type of IP addresses with Jaccard distance 
% (Eq.~\ref{eq:jaccard-distance-coverage}) in parenthesis}
% \label{fig:coverage-ip-typee}
% \vspace{-3mm}
%\end{figure}

\paragraph{Deeper investigation on country changes}

\begin{figure}[h]
 \centering
\includegraphics[width=0.40\linewidth]{figures/whois_ripe_root_cause.pdf}
 \vspace{-3mm}
 \caption{Jaccard distance between countries in \maxmind and whois
 for IP addresses with country changes versus random IP addresses.}
   \label{fig:who-is-correlation}
\end{figure}

As alluded to earlier,
there is a common belief that \maxmind, and other geolocation databases, 
use in part registry information from the whois database.
The IP addresses that changed country are ideal candidates to evaluate
this belief, as historical whois information is available. 
Among the Regional Internet Registries, RIPE provides an API
to the historical whois data and their updates~\cite{whowas}.

We build two IP sets to find if there is any correlation between 
the countries reflected in the 
\maxmind and whois databases. 
The first set, ``multiple,'' is composed of 90,475 randomly selected IP addresses 
that have more than two countries in 2019 and 
that are managed by RIPE. The second set, ``control,'' is composed of 99,989
randomly selected IP addresses that are managed by RIPE.  For each
set, we lookup the \maxmind country-level location, 
as well as the whois registry reported country, of each IP address.

Fig.~\ref{fig:who-is-correlation} shows the Jaccard distance between
the countries found from \maxmind versus whois for the control and
multiple IP sets.
This plot shows that on the control set, 96\% of the IP addresses have a 
Jaccard distance of 0, meaning that \maxmind and whois perfectly match.
However, for the multiple set only 3\%
of the IP addresses have a Jaccard distance of 0. Notice that 
we show the multiple set for different values of maximum prevalence 
(Eq.~\ref{eq:max-prevalence-ip}). This shows that even when 
there is no dominant country (maximum prevalence $\leqslant$ 0.5),
the \maxmind and whois countries are not aligned.  
Again, we conclude that country changes in the \maxmind database are not correlated
with the whois database. 

\paragraph{\textbf{Lesson}}
The common belief that \maxmind database gets their geolocation 
information from whois registry databases does not hold for IP addresses 
geolocated to multiple countries.


